Measurement of the top quark-pair production cross section with ATLAS in pp collisions at $\sqrt{s}=7\TeV$

A measurement of the production cross-section for top quark pairs($\ttbar$) in $pp$ collisions at $\sqrt{s}=7 \TeV$ is presented using data recorded with the ATLAS detector at the Large Hadron Collider. Events are selected in two different topologies: single lepton (electron $e$ or muon $\mu$) with large missing transverse energy and at least four jets, and dilepton ($ee$, $\mu\mu$ or $e\mu$) with large missing transverse energy and at least two jets. In a data sample of 2.9 pb-1, 37 candidate events are observed in the single-lepton topology and 9 events in the dilepton topology. The corresponding expected backgrounds from non-$\ttbar$ Standard Model processes are estimated using data-driven methods and determined to be $12.2 \pm 3.9$ events and $2.5 \pm 0.6$ events, respectively. The kinematic properties of the selected events are consistent with SM $\ttbar$ production. The inclusive top quark pair production cross-section is measured to be $\sigmattbar=145 \pm 31 ^{+42}_{-27}$ pb where the first uncertainty is statistical and the second systematic. The measurement agrees with perturbative QCD calculations.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = main_unified

default: testlatex

testlatex:
	latex  ${BASENAME}; \
	latex  ${BASENAME}; \
	bibtex ${BASENAME}; \
	latex  ${BASENAME}; \
	latex  ${BASENAME}
	dvips  ${BASENAME} -o ${BASENAME}.ps
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}; \
	pdflatex  ${BASENAME}; \
	bibtex    ${BASENAME}; \
	pdflatex  ${BASENAME}; \
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


